Deconstructing Categorization in Visualization Recommendation: A Taxonomy and Comparative Study

Visualization recommendation (VisRec) systems provide users with suggestions for potentially interesting and useful next steps during exploratory data analysis. These recommendations are typically organized into categories based on their analytical actions, i.e., operations employed to transition from the current exploration state to a recommended visualization. However, despite the emergence of a plethora of VisRec systems in recent work, the utility of the categories employed by these systems in analytical workflows has not been systematically investigated. Our paper explores the efficacy of recommendation categories by formalizing a taxonomy of common categories and developing a system, Frontier, that implements these categories. Using Frontier, we evaluate workflow strategies adopted by users and how categories influence those strategies. Participants found recommendations that add attributes to enhance the current visualization and recommendations that filter to sub-populations to be comparatively most useful during data exploration. Our findings pave the way for next-generation VisRec systems that are adaptive and personalized via carefully chosen, effective recommendation categories.

==> contributions.tex <==

\doris{It would also be useful to add some findings here.}


Our contributions are summarized as follows:
\begin{tight_itemize}
\item Drawing from visual analytics recommendations literature, we introduce a list of common facet categories for visualization recommendations. 
\item We introduce a system \textit{Frontier} along with its motivating design principles, interface design, and system architecture to explore facet categories. The facets provide visualization recommendations that serve as ``one-step away'' guideposts with respect to the user's current view.
% as shown in a user's workflow vignette in Figure \ref{fig:teaser}, where he made use of the facets to gain contextual insights regarding the data distributions, finding data subsets that explain an observed piecewise correlation, and discover salient data clusters. \melanie{moved this up; shouldn't be appearing for the first time in contributions}
\item We present a mixed methods user study focused on exploratory data analysis to understand how users employ visualization recommendations and how the facet categories influence those workflows.
\item Lastly, we discuss design implications for visualization tools that employ facets to support data exploration. 
\end{tight_itemize}






==> landscape_table.tex <==
%!TEX root = main.tex
\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
\begin{table}[ht!]
\vspace*{-5pt}
\centering
  \begin{tabular}{|C{2.4cm}|C{.9cm}|C{1.1cm}|C{1.1cm}|C{1.1cm}|C{0.8cm}|C{0.8cm}|C{1cm}|C{1.3cm}|C{1.1cm}|C{1.5cm}|}
        \hline
       \small{ \textbf{Action Type}} & \color{crimson}   \small{\textbf{Frontier}} & \centering\small{\textbf{Voyager}\cite{Wongsuphasawat2016}} & \centering    \small{\textbf{Voyager2}\cite{Wongsuphasawat2017}} & \centering    \small{\textbf{DataSite} \cite{datasite}} & \centering    \small{\textbf{DIVE} \cite{hu2018dive}} & \centering    \small{\textbf{Duet} \cite{law2019duet}} & \centering    \small{\textbf{SEEDB} \cite{Vartak2015}} & \centering    \small{\textbf{Zenvisage} \cite{zenvisage}} & \centering    \small{\textbf{VisPilot} \cite{Lee:2019} }& \centering    \small{\textbf{ScagExplorer} ~\cite{Dang:2014}} \tabularnewline
        \hline 
        \small{Distribution} & \cellcolor{cambridgeblue}\cmark & \cellcolor{cambridgeblue}\cmark & \cellcolor{cambridgeblue}\cmark & \xmark & \cellcolor{cambridgeblue}\cmark & \xmark & \xmark & \xmark & \xmark & \xmark  \\
        \hline
         \small{Correlation} & \cellcolor{cambridgeblue}\cmark  & \xmark & \cellcolor{cambridgeblue}\cmark & \cellcolor{cambridgeblue}\cmark  & \cellcolor{cambridgeblue}\cmark & \xmark & \xmark &\xmark & \xmark & \cellcolor{cambridgeblue}\cmark \\
        \hline
         \small{Enhance} & \cellcolor{cambridgeblue}\cmark & \cellcolor{cambridgeblue}\cmark & \cellcolor{cambridgeblue}\cmark & \xmark & \cellcolor{cambridgeblue}\cmark & \xmark & \xmark & \xmark & \xmark & \xmark  \\
        \hline
         \small{Generalize (attribute)} & \cellcolor{cambridgeblue}\cmark  & \xmark & \xmark & \xmark & \cellcolor{cambridgeblue}\cmark  & \xmark & \xmark & \xmark & \xmark & \xmark \\
         \hline
          \small{Generalize (value)} & \cellcolor{cambridgeblue}\cmark  & \xmark & \xmark & \xmark & \cellcolor{cambridgeblue}\cmark  & \xmark & \xmark & \xmark & \xmark & \xmark \\
         \hline
         \small{Pivot} & \cellcolor{cambridgeblue}\cmark  & \xmark & \xmark & \xmark & \cellcolor{cambridgeblue}\cmark & \xmark & \xmark & \xmark & \xmark & \xmark  \\
         \hline
         \small{Filter (add)} & \cellcolor{cambridgeblue}\cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cellcolor{cambridgeblue}\cmark & \xmark\\
         \hline
         \small{Filter (swap)} & \cellcolor{cambridgeblue}\cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cellcolor{cambridgeblue}\cmark & \xmark & \xmark\\
         \hline
        \small{Similarity (diff)} & \cellcolor{cambridgeblue}\cmark  & \xmark & \xmark & \xmark & \xmark & \cellcolor{cambridgeblue}\cmark & \cellcolor{cambridgeblue}\cmark & \xmark & \xmark & \xmark \\
       \hline
        \small{Similarity (sim)} & \cellcolor{cambridgeblue}\cmark  & \xmark & \xmark & \xmark & \xmark & \cellcolor{cambridgeblue}\cmark & \xmark & \cellcolor{cambridgeblue}\cmark & \xmark & \xmark \\
         \hline
    \end{tabular}
    \caption{Research landscape of actions in visual recommendation systems. The table encompassing 17 systems is found in the supplementary material.}
    \label{tab:landscape}
    \vspace*{-5pt}
\end{table}

==> model.tex <==
\subsection{Model}
\par As described in the previous section, our recommendation model is inspired by hub and spoke model from web search (CITE). We model the space of possible visualizations as a hypergraph G, where the nodes are attributes and values. For any given dataset, we consider node entities consisting of attributes (A-nodes) and their corresponding values (V-nodes). A-nodes corresponding to categorical attributes can contain V-nodes, as illustrated in Figure~\ref{graph_example} where the A-node \texttt{Class} node contains V-nodes \texttt{1},\texttt{2}, \texttt{3}\footnote{Note that this formulation can be extended to numerical attributes with a binning parameter, but for clarity we do not cover this in our work.}. 
\par Given the initial lattice composed of A and V nodes constructed from the dataset, we further extend the lattice based on a set of user selections S. S represents the attributes or values that a user is interest or disinterested in. In the Figure~\ref{graph_example} example, the user is interested in the attribute \texttt{Fare} and \texttt{NumberSurvived}. Based on these user selections, we create S-nodes representating all combinations of entites in S. For example, the S-nodes in the example are \{\texttt{Fare} AND \texttt{NumberSurvived}\}, \{\texttt{Fare}\} and \{\texttt{NumberSurvived}\} (displayed as starred node, the latter two S-nodes are occluded since they are also F-nodes, described next).
\par Given a lattice representation of all current user selections, we generate facets (F-nodes) by looking at all possible single-modifications to the created S-nodes. Modifications to S-nodes can be characterized by two motion paths:
\begin{enumerate}
	\item \textbf{Climb}: Adding or Removing an attribute or filter
	\item \textbf{Crawl}: Changing an attribute or filter
\end{enumerate}
The collection of visualizations in each facet is characterized by the wildcards (inspired by ~\cite{Wongsuphasawat2016}), with \texttt{A?} iterating through the collection of attributes or \texttt{F?} iterating through the collection of filters. Additionally,wildcards on filter values \texttt{V?} iterate through all possible values that could be adopted for the specified attribute(e.g., \texttt{Class=V?} translates to \texttt{Class=1}, \texttt{Class=2}, \texttt{Class=3})
\par To select the best facets to be displayed to the user, we iterate through the collection of visualizations in each facet to compute a score. Some notion of relevancy of the facet is also computed at the F-node level. We take the maximum score across all visualization of a particular F-node as the score of that F-node, then perform ranking across the possible F-nodes at any particular state.
\begin{figure}[ht!]
  \centering
  \includegraphics[width=0.95\linewidth]{figures/graph_example.png}
  \caption{Example of a graph in our faceted model for visualizations. The user has expressed interest in \texttt{Fare} and \texttt{NumberSurvived}. The star nodes are S-nodes and green rectangular nodes are F-nodes representing potential facets. Note that some F-nodes are also S-nodes.}
  \label{graph_example}
\end{figure}

==> objective_tbl.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \begin{tabular}{|p{0.2cm}|p{0.2cm}|p{0.33cm}|p{6.5cm}|}
% \hline
% \small{|D|}  & \small{|M|}  & \small{|F|} & Objective                                                                                                                                                       \\ \hline
% \multirow{2}{*}{1} & \multirow{2}{*}{0} & 0                    & Skewness~\cite{demiralp2017foresight}.                                                                               \\ \cline{3-4} 
%                    &                    & 1                    & Deviation of filtered distribution from the overall.                                                                                                            \\ \hline
% \multirow{2}{*}{0} & \multirow{2}{*}{1} & 0                    & Aggregated frequency counts of the distribution~\cite{datasite}.                                                                                                \\ \cline{3-4} 
%                    &                    & 1                    & Deviation of filtered distribution from the overall.                                                                                                            \\ \hline
% \multirow{2}{*}{1} & \multirow{2}{*}{1} & 0                    & Unevenness of bar chart: deviation from the max-entropy distribution~\cite{Sarawagi2001, Sarawagi1998}. Computed only if cardinality < 40.                      \\ \cline{3-4} 
%                    &                    & 1                    & Deviation of the bar chart from the overall. Computed only if cardinality<40.                                                                                   \\ \hline
% \multirow{2}{*}{0} & \multirow{2}{*}{2} & 0                    & Mutual information: capture both linear and non-linear relationships between measures~\cite{Murphy2012}                                                         \\ \cline{3-4} 
%                    &                    & 1                    & Monotonicity: scagnostic measure that determines linear functional dependence between two measures~\cite{wilkinson2005graph}.                                        \\ \hline
% \multirow{2}{*}{2} & \multirow{2}{*}{1} & 0                    & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Unevenness between the ratios in each group \\ based on colored dimension.\end{tabular}}                             \\ \cline{3-3}
%                    &                    & 1                    &                                                                                                                                                                 \\ \hline
% \multirow{2}{*}{1} & \multirow{2}{*}{2} & 0                    & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Cluster separation based on colored dimension~\cite{Sedlmair2012}. \\ Computed only if cardinality<10.\end{tabular}} \\ \cline{3-3}
%                    &                    & 1                    &                                                                                                                                                                 \\ \hline
% \end{tabular}
% \caption{Table of the recommendation objectives in \frontier for visualizations recommendation as part of the operational category. }
% \label{tbl:objective}
% \end{table}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
    \begin{tabular}{|p{0.2cm}|p{0.2cm}|p{0.33cm}|p{12cm}|}
    \hline
    \small{|D|}  & \small{|M|}  & \small{|F|} & Objective                                                                                                                                                       \\ \hline
    \multirow{2}{*}{1} & \multirow{2}{*}{0} & 0                    & Skewness~\cite{demiralp2017foresight}.                                                                               \\ \cline{3-4} 
                       &                    & 1                    & Deviation of filtered distribution from the overall.                                                                                                            \\ \hline
    \multirow{2}{*}{0} & \multirow{2}{*}{1} & 0                    & Aggregated frequency counts of the distribution~\cite{datasite}.                                                                                                \\ \cline{3-4} 
                       &                    & 1                    & Deviation of filtered distribution from the overall.                                                                                                            \\ \hline
    \multirow{2}{*}{1} & \multirow{2}{*}{1} & 0                    & Unevenness of bar chart: deviation from the max-entropy distribution~\cite{Sarawagi2001, Sarawagi1998}. Computed only if cardinality < 40.                      \\ \cline{3-4} 
                       &                    & 1                    & Deviation of the bar chart from the overall. Computed only if cardinality<40.                                                                                   \\ \hline
    \multirow{2}{*}{0} & \multirow{2}{*}{2} & 0                    & Mutual information: capture both linear and non-linear relationships between measures~\cite{Murphy2012}                                                         \\ \cline{3-4} 
                       &                    & 1                    & Monotonicity: scagnostic measure that determines linear functional dependence between two measures~\cite{wilkinson2005graph}.                                        \\ \hline
    \multirow{2}{*}{2} & \multirow{2}{*}{1} & 0                    & Unevenness between the ratios in each group based on colored dimension.                         \\ \cline{3-3}
                       &                    & 1                    &                                                                                                                                                                 \\ \hline
    \multirow{2}{*}{1} & \multirow{2}{*}{2} & 0                    & Cluster separation based on colored dimension~\cite{Sedlmair2012}. Computed only if cardinality<10.\\ \cline{3-3}
                       &                    & 1                    &                                                                                                                                                                 \\ \hline
    \end{tabular}
    \caption{Table of the recommendation objectives in \frontier for visualizations recommendation as part of the operational category. }
    \label{tbl:objective}
    \end{table}
